ScaleQC: A Scalable Framework for Hybrid Computation on Quantum and Classical Processors

Quantum processing unit (QPU) has to satisfy highly demanding quantity and quality requirements on its qubits to produce accurate results for problems at useful scales. Furthermore, classical simulations of quantum circuits generally do not scale. Instead, quantum circuit cutting techniques cut and distribute a large quantum circuit into multiple smaller subcircuits feasible for less powerful QPUs. However, the classical post-processing incurred from the cutting introduces runtime and memory bottlenecks. Our tool, called ScaleQC, addresses the bottlenecks by developing novel algorithmic techniques including (1) a quantum states merging framework that quickly locates the solution states of large quantum circuits; (2) an automatic solver that cuts complex quantum circuits to fit on less powerful QPUs; and (3) a tensor network based post-processing that minimizes the classical overhead. Our experiments demonstrate both QPU requirement advantages over the purely quantum platforms, and runtime advantages over the purely classical platforms for benchmarks up to 1000 qubits.

==> text/Approximate_Output_Fidelity.tex <==
\subsection{Runtime and Accuracy Trade-offs of Approximate Outputs}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/compare_states_merging.pdf}
    \caption{Accuracy and runtime comparisons for a $24$-qubit benchmark circuit with $0$ degree of connection.
    Every data point is the average of $5$ random trials.
    Cut\_S and Cut\_SM use the same samples for each trial.
    Cut\_SM runs to completion with $2^{10}$ bins per recursion.
    Given enough recursions, states merging does not degrade the output accuracy.
    States merging runs slower for medium sized benchmarks but will scale to arbitrary sized circuits.
    The computation cost of optimal sampling is sub-linear with respect to accuracy.}
    \label{fig:compare_states_merging}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/compare_sampling.pdf}
    \caption{Accuracy and runtime comparisons for a $24$-qubit benchmark circuit with $0.5$ degree of connection.
    The example has $5$ cuts hence $4^5$ edge bases without sampling.
    Cut\_SM automatically chooses the $2$ most important edge bases.
    Cut\_SM and Cut\_M are both capped at $2^{10}$ bins per recursion.
    Optimal sampling trades large runtime improvement for negligible accuracy loss.
    }
    \label{fig:compare_sampling}
\end{figure}

While NISQ QPU noise is the bottleneck for producing accurate results nowadays,
we anticipate ScaleQC applications to become much more useful with medium sized noise resilient QPUs.
Thus, we focus on the non-QPU sources of approximations and inaccuracies
from both optimal sampling and states merging.
Furthermore, the possible values of the approximation error depends on the ground truth $P$ itself,
hence approximation errors across different circuits do not directly compare.
As a result, each experiment only compares the error for a single benchmark circuit.

In addition, as Section~\ref{sec:compute_graph_contraction} mentions,
while ScaleQC produces accurate outputs,
the results are usually in a different qubit order due to the compute graph contraction orders.
For practical purposes,
ScaleQC helps locate a very small subset of solution states and can easily convert the qubit orders for the solution states found.
However, doing so for all $2^n$ states can be slow.
Hence the experiments use $24$-qubit benchmark circuits.

Figure~\ref{fig:compare_states_merging} compares Cut\_S and Cut\_SM for various number of samples.
For this experiment only, we append $5$ $Hadamard$ gates to arbitrary qubits in the $BV$ benchmark in order to arbitrarily encode more solution states.
This temporary modification more clearly demonstrates the effect of optimal sampling.

Cut\_SM combines states merging in addition to Cut\_S.
Given enough number of recursions,
Cut\_SM achieves similar accuracy as Cut\_S.
Although Cut\_SM is slower than Cut\_S for medium sized circuits,
it works for arbitrary sized benchmarks because it circumvents the memory requirements via merging.

The computation cost of optimal sampling is only sub-linear with respect to approximation errors.
The approximation errors decrease polynomial for Cut\_S as the number of samples increases.
Meanwhile, the runtime of Cut\_S does not increase as much.
Using more samples simply re-picks the most important ones more often.
Since the runtime only depends on the number of distinct samples,
more samples decrease the errors while maintaining the runtime.

Figure~\ref{fig:compare_sampling} compares Cut\_M and Cut\_SM for various number of recursions.
The errors decrease rapidly as more recursions are used.
The exact number of recursions is not directly controlled,
as states merging also terminates when all the solution states are found.
Hence the number of recursions in the figure appears irregular.
For each of the $1$, $10$, $20$, $50$ and $100$ max number of recursions,
we repeat $5$ trials.
Cut\_M computes all $4^5$ edge bases and is able to produce nearly the exact output after around $30$ recursions.

Cut\_SM further combines optimal sampling with $2^{10}$ samples and produces quite similar accuracy.
Experiment shows that out of the $2^{10}$ total samples picked by Cut\_SM,
only $2$ are distinct.
Thus, Cut\_SM is able to ignore a lot of the edge bases that do not affect the output
and only computes the ones that matter.
As a result, optimal sampling trades large runtime improvement for little accuracy loss.

==> text/Arbitrary_Sampling.tex <==
\subsection{Sampling with Arbitrary Probability}\label{sec:arbitrary_prob}
\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetAlgoLined
    \caption{ARBITRARY SAMPLING}\label{alg:arbitrary_sampling}
    \KwIn{Number of samples $c$.
    Sampling probability $\{q_k\}_{k=1}^{4^K}$ such that $\sum_{k=1}^{4^K}q_k=1$.}
    Initialize a counter $\lambda_k=0$, $\forall k\in\{1,\ldots,4^K\}$\;
    \For{$t=1\to c$}{
        Pick $k_t\in\{1,\ldots,4^K\}$ with probability $P[k_t=k]=q_k$ independently and with replacement\;
        $\lambda_{k_t}\gets\lambda_{k_t}+1$\;
    }
    $\widetilde{P}\equiv\sum_{k}\lambda_{k}\otimes_{i=1}^{n_C}p_{i,k}/cq_{k}$\;
\end{algorithm}
The actual computation of the compute graph contraction process is in fact matrix multiplications.
Every column of the leading matrix and every row of the trailing matrix are constructed from the subcircuit entries.
As such, approximating the result is similar with the Monte Carlo approximations of matrix products~\cite{drineas2006fast}.
Instead of computing the exact result by considering every leading column and its corresponding trailing row,
we can sample an important subset of the matrix elements to include in the computations to trade accuracy with runtime.
Specifically, we aim to minimize the approximation error, defined as
\begin{equation}
    \epsilon\equiv\left|P-\widetilde{P}\right|^2\label{eq:approximation_error}
\end{equation}
where $P$ is the ground truth of the quantum circuit and $\widetilde{P}$ is its approximation.

Algorithm~\ref{alg:arbitrary_sampling} shows a sampling algorithm with arbitrary sampling probabilities,
which samples a total of $c$ edge bases.
Following similar proofs from~\cite{drineas2006fast},
Lemma~\ref{lemma:arbitrary_sampling} shows the expectation and approximation error guarantees.
\begin{lemma}\label{lemma:arbitrary_sampling}
For any valid probability distributions, define $\widetilde{P}$ according to Algorithm~\ref{alg:arbitrary_sampling} as an approximation to $P$.
The expectation of any quantum state $\forall j\in\{1,\ldots,2^n\}$
and the expectation of the overall approximation error are
    \begin{eqnarray}
        \mathbb{E}[\widetilde{P}_j]&=&P_j\label{eq:arbitrary_expectation}\\
        \mathbb{E}[\epsilon]&=&\frac{1}{c}\sum_{k=1}^{4^K}\frac{1}{q_k}\prod_{i=1}^{n_C}|p_{i,k}|^2-\frac{1}{c}|P|^2\label{eq:arbitrary_error}
    \end{eqnarray}
\end{lemma}

Equation~\ref{eq:arbitrary_expectation} shows that the expectation of the result is independent of the choice of the sampling probabilities.
In fact, Algorithm~\ref{alg:arbitrary_sampling} always converges to the exact values even for uniform sampling.
However, Equation~\ref{eq:arbitrary_error} shows that the expectation of the approximation errors depends on the sampling probabilities.

Note that the number of samples $c$ is allowed to exceed $4^K$.
Sampling the same summation term more than once just equates to multiply it by its frequency.
Since the compute graph contraction process does not compute $\widetilde{P}$ term by term,
this does not add extra compute overhead.
In fact, our experiments using optimal sampling show that in many cases,
the vast majority of the terms do not matter and are never picked,
even when $c$ is large.

==> text/Essential_Sampling.tex <==
\subsection{Essential Sampling}
\begin{algorithm}[ht]
\SetAlgoVlined
Initialize $\widetilde{P}=0\in\mathbb{R}^{2^n}$.\\
Relabel $j\in\{1,\ldots,n_C\}$, where $C_j$ has a manageable number of distinct elements, as $C_1$.\\
Use QPUs to evaluate $C_{1,k}$, $\forall k$.\\
Choose $c\in\mathbb{Z}^+$ such that $1\leq c\leq4^K$.\\
Choose $\{p_k\}_{k=1}^{4^K}$ such that $p_k=\frac{|C_{1,k}|}{\sum_{k'}|C_{1,k'}|}$.\\
\For{$t=1$ to $c$}{
Pick $k_t\in\{1,\ldots,4^K\}$ with probability $P[k_t=k]=p_k$ independently and with replacement.\\
Use QPUs to evaluate $C_{i,k_t}$, $i\in\{2,\ldots,n_C\}$.\\
Compute $\otimes_{i=1}^{n_C}C_{i,k_t}/cp_{k_t}$ and add to $\widetilde{P}$.
}
Return $\widetilde{P}$.
\caption{ESSENTIAL SAMPLING (ES)}
 \label{alg:essential_sampling}
\end{algorithm}
Uniform sampling is easy to implement but may have poor approximation errors. Optimal sampling has the minimum approximation errors, but needs to satisfy the implementation prerequisites. Algorithm~\ref{alg:essential_sampling} provides a balanced trade-off. Essential sampling samples the summation terms based on the output of one of the ``narrow'' subcircuits. A ``narrow'' subcircuit has a manageable number of distinct elements so that a non-uniform sampling distribution can be efficiently computed.

Substituting the probabilities into Equation~\ref{eq:GR_error} gives the expected approximation error of essential sampling.
\begin{eqnarray*}
\mathbb{E}\left[|P-\widetilde{P}|^2\right]_{\text{essential}}&=&\frac{1}{c}\sum_{k=1}^{4^K}\frac{\sum_{k'}|C_{1,k'}|}{|C_{1,k}|}\prod_{i=1}^{n_C}|C_{i,k}|^2-\frac{1}{c}|P|^2\\
&=&\frac{1}{c}\sum_{k,k'=1}^{4^K}\frac{|C_{1,k'}|}{|C_{1,k}|}\prod_{i=1}^{n_C}|C_{i,k}|^2-\frac{1}{c}|P|^2
\end{eqnarray*}

Compared to uniform sampling, ES guarantees a lower approximation error. Since ES intentionally picks a subcircuit with a manageable number of distinct elements, the corresponding sampling probabilities can be efficiently computed. In addition, the QPUs only need to fully evaluate one subcircuit and evaluate the rest on the fly only if picked. Therefore, ES uses information of one subcircuit to automatically extract the essential variations of other subcircuits.

==> text/Experiments_Summary.tex <==
\subsection{Summary of Experiments}\label{sec:experiments_summary}
Table~\ref{table:experiments} summarizes the four sets of experiments to evaluate the ScaleQC framework.

The first set of experiments use medium benchmarks where a full state circuit output still fits in the memory.
This cutoff depends on the particular classical backend available to the users,
we use $30$ qubits as the cutoff in this paper.
However, since each qubit doubles the memory requirement,
there is little value in pushing this cutoff point to the extreme.
Classical and Cut produce the full state solution states with $P_{full}$.
We compare the full-state runtime of the two.

The second set of experiments use large benchmarks whose full state space no longer fits in the memory.
ScaleQC with states merging becomes necessary in this regime.
We cannot analyze the accuracy in this regime as neither QPUs or CPUs nowadays can quickly produce reliable large subcircuits outputs.
We hence compare the runtime of Cut\_M and the extrapolated runtime of Classical to demonstrate the scalability of ScaleQC.

The third set of experiments use the same large benchmarks to study the quantum resources requirements.
We compare the quantum area requirements of Quantum and Cut\_M to demonstrate the quantum resources advantages of ScaleQC.

The fourth set of experiments use medium benchmarks and aims at demonstrating the effectiveness of optimal sampling and states merging.
We compare Cut\_S, Cut\_M and Cut\_SM for runtime versus accuracy trade-offs.

==> text/Optimal_Sampling.tex <==
\section{Optimal Sampling}\label{sec:optimal_sampling}
Optimal sampling is the first amplitude-aware sampling in any quantum circuit evaluations works, classical or quantum.
Furthermore, this paper establishes the optimality of the algorithm.
On the other hand,
the state-of-the-art classical simulation work~\cite{liu2021closing} uses sampling that is
(1) applied in a quite different context,
(2) merely random,
(3) without any error bounds guarantees, and
(4) narrowly applies to random circuits such as Supremacy and will not work for all other benchmarks used in our paper.

While ScaleQC can perform exact reconstructions of the input quantum circuit by computing all the subcircuit entries,
some subcircuit entries affect the output accuracy much more significantly than the others.
As a result, by intelligently selecting and only computing the most contributing subcircuit entries,
optimal sampling retains the closest approximation while performing the least amount of computation possible.

Section~\ref{sec:arbitrary_prob} first introduces the sampling framework for any arbitrary sampling probability,
and derives the dependence of approximation errors on the sampling probability.
Section~\ref{sec:optimal_prob} then shows how to choose the optimal sampling probability to minimize the approximation errors with a sub-linear computation cost.

\input{text/Arbitrary_Sampling}

\subsection{Sampling with Optimal Probability}\label{sec:optimal_prob}
Optimal sampling probability aims to intelligently select the important terms more often.
Lemma~\ref{lemma:optimal_sampling} shows the optimal sampling probabilities in terms of minimizing the expected approximation error $\epsilon$ for a given number of samples $c$.
\begin{lemma}
Define $\widetilde{P}$ according to Algorithm~\ref{alg:arbitrary_sampling} as an approximation to $P$,
then the optimal probability distribution that minimizes this expected approximation error is
\begin{equation}
    q_k=\frac{\prod_{i=1}^{n_C}|p_{i,k}|}{\sum_{k'=1}^{4^K}\prod_{i=1}^{n_C}|p_{i,k'}|}\label{eq:optimal_probability}
\end{equation}
It follows that the optimal expected approximation error decreases linearly with number of samples
\begin{equation}
    \mathbb{E}[\epsilon]_{\text{optimal}}=\frac{1}{c}\left(\sum_{k=1}^{4^K}\prod_{i=1}^{n_C}|p_{i,k}|\right)^2-\frac{1}{c}|P|^2\label{eq:optimal_error}
\end{equation}
\label{lemma:optimal_sampling}
\end{lemma}

The proof closely follows from the matrix product proofs in~\cite{drineas2006fast}.
Optimal sampling guarantees the best possible $\epsilon$ for a given number of samples.
Since optimal sampling chooses the edge bases with replacement,
selecting $c$ samples usually requires to compute much fewer than $c$ distinct edge bases.
This is especially beneficial if the optimal probabilities concentrate on just a few edge bases.
In fact, this demonstrates the advantage of optimal sampling over exact computation in its ability to intelligently select the edge bases that matter the most.
Equation~\ref{eq:optimal_error} shows that the error decreases linearly with the number of samples $c$.
However, since the actual amount of computation required only depends on the number of distinct samples,
optimal sampling in fact provides a sub-linear computation complexity to reduce the approximation errors.

An intuitive understanding of the optimal sampling method is that
a particular subcircuit output contributes more to the quantum state probability if its output has larger magnitudes.
Optimal sampling hence seeks to only compute the subcircuit entries with higher magnitudes.
Optimal sampling significantly reduces the amount of computation,
and offers an optional trade-off versus the exact computation.

==> text/Programming_Techniques.tex <==
\section{Programming Techniques}\label{sec:programming_techniques}
\wtnote{needs updates}
The bulk of the postprocessing is taking the outer products among the subcircuit outputs.
This is essentially computing the matrix-matrix multiplications.
We use the state-of-the-art computing kernels from the Intel Math Kernel Library (MKL)~\cite{wang2014intel} compiled in $C$ for the best performance on Intel CPUs.

In addition, the Qiskit quantum package generates QPU data in Python,
which introduces extra data transfer overhead to utilize the MKL kernels.
We use Cython~\cite{behnel2010cython} to wrap the MKL routines with a Python interface to directly operate on Python data types.
The wrapper significantly reduces the data transfer overhead.

Furthermore, the matrices span a wide range of sizes and densities,
which significantly affect the MKL kernel performances.
Therefore, we wrapped and benchmarked the performances of dense-dense (\textit{cblas\_sgemm} routine),
sparse-dense/dense-sparse (\textit{mkl\_sparse\_s\_mm} routine),
and sparse-sparse (\textit{mkl\_sparse\_s\_spmmd} routine) MKL matrix multiplication routines
for different combinations of densities and sizes.
We constructed a KD Tree using the benchmark results for fast selections of routines based on the input matrices characteristics.
The benchmarking is an optional but useful step to enhance the compute runtime.

Via these programming techniques,
we reduce the compute graph contraction runtime to generally less than half of the ScaleQC runtime.
Our benchmarking shows that the cut location process becomes the bottleneck but is nonetheless very fast.

==> text/Quantum_Classical_Tradeoff.tex <==
\subsection{Quantum and Classical Resources Tradeoff}
\wtnote{Sweep the max load factor for an example benchmark}

==> text/Uniform_Sampling.tex <==
\subsection{Uniform Sampling}
\begin{algorithm}[ht]
\SetAlgoVlined
Initialize $\widetilde{P}=0\in\mathbb{R}^{2^n}$.\\
Choose $c\in\mathbb{Z}^+$ such that $1\leq c\leq4^K$.\\
Choose $\{p_k\}_{k=1}^{4^K}$ such that $p_k=\frac{1}{4^K}$.\\
\For{$t=1$ to $c$}{
Pick $k_t\in\{1,\ldots,4^K\}$ with probability $P[k_t=k]=p_k$ independently and with replacement.\\
Use QPUs to evaluate $C_{i,k_t}$, $\forall i\in\{1,\ldots,n_C\}$.\\
Compute $\otimes_{i=1}^{n_C}C_{i,k_t}/cp_{k_t}$ and add to $\widetilde{P}$.
}
Return $\widetilde{P}$.
\caption{UNIFORM SAMPLING (US)}
 \label{alg:uniform_sampling}
\end{algorithm}
Algorithm~\ref{alg:uniform_sampling} uniformly samples the summation terms. Uniform sampling is the easiest to implement and does not require any prior knowledge on the exact entries of the output of the subcircuits. This carries two benefits: (1) there is no need to compute the individual $p_k$ for the summation terms, which can be difficult due to the large number of $k$; and (2) the QPUs only need to evaluate the subcircuit variations that get picked, instead of having to evaluate everything.

Substituting uniform probabilities into Equation~\ref{eq:GR_error} gives the approximation error of uniform sampling.
\begin{equation}
\mathbb{E}\left[|P-\widetilde{P}|^2\right]_{\text{uniform}}=\frac{4^K}{c}\sum_{k=1}^{4^K}\prod_{i=1}^{n_C}|C_{i,k}|^2-\frac{1}{c}|P|^2\label{eq:uniform_error}
\end{equation}

==> text/__latexindent_temp.tex <==
\section{Compute Graph Contraction}\label{sec:compute_graph_contraction}
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/contraction_step_1.pdf}
        \caption{Contracting subcircuits $2,3$.}
        \label{fig:contraction_step_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/contraction_step_2.pdf}
        \caption{Contracting subcircuit $1$ with $2,3$.}
        \label{fig:contraction_step_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/contraction_step_3.pdf}
        \caption{Contracting subcircuit $4$ with $1,2,3$.}
        \label{fig:contraction_step_3}
    \end{subfigure}
       \caption{The figure shows the compute graph generated from cutting a $25$-qubit random benchmark circuit (Section~\ref{sec:benchmarks}) into $12$-qubit subcircuits and roughly half the circuit size.
       Some of the edges have the same origin and destination subcircuits,
       represented by a slash on the edges.
       Each subcircuit also has different number of qubits,
       hence different lengths of output vectors.
       The subfigures show the best contraction order of $3,2,1,4$.
       The dashed edges are the contraction edges in each step.
       The double edges are the relevant edges in each step.
       The solid edges are the irrelevant edges in each step.
       The last contraction merges all the subcircuits into a single node (not shown) and concludes the compute graph computation.}
       \label{fig:compute_graph_contraction_example}
\end{figure}

\begin{algorithm}[t]
    \caption{Compute Graph Contraction}\label{alg:compute_graph_contraction}
    \textbf{INPUT}
    Compute graph $G$.
    Contraction order $L$.
    \begin{algorithmic}[1]
        \State $i\gets1$
        \While{$i<\#G.nodes$}
            \State Initialize an empty \textit{data\_buffer}, \textit{next\_data\_buffer}
            \State \textit{leading\_subcircuit} $\gets L[i]$
            \State \textit{contracted\_subcircuits} $\gets L[:i]$
            \State \multiline{%
            \textit{contraction\_edges} $\gets$ edges connecting the \textit{leading\_subcircuit} and the \textit{contracted\_subcircuits}}
            \State \multiline{%
            \textit{leading\_edges} $\gets$ edges connecting only the \textit{leading\_subcircuit}}
            \State \multiline{%
            \textit{trailing\_edges} $\gets$ edges connecting only the \textit{contracted\_subcircuits}}
            \For{$e\in\{I,X,Y,Z\}^{\#\textrm{\textit{leading\_edges}}+\#\textrm{\textit{trailing\_edges}}}$}
                \State $e_l\gets e[:\#\textrm{\textit{leading\_edges}}]$
                \State $e_t\gets e[\#\textrm{\textit{leading edges}}:]$
                \State \multiline{%
                Assign the leading edge bases $e_l$ to the \textit{leading edges}}
                \State \multiline{%
                Assign the trailing edge bases $e_t$ to the \textit{trailing edges}}
                \State \multiline{%
                Initialize the \textit{leading matrix} as a zero matrix of shape $(2^{G.sizes[L[i]]},4^{\#\textrm{contraction edges}})$}
                \State \multiline{%
                Initialize the \textit{trailing matrix} as a zero matrix of shape $(4^{\#\textrm{contraction edges}},2^{\sum G.sizes[L[:i]]})$}
                \State $j\gets0$
                \For{$[e_c]\in\{I,X,Y,Z\}^{\#\textrm{contraction edges}}$}
                    \State \multiline{%
                    Assign the contraction edge bases $[e_c]$ to the \textit{contraction edges}}
                    \State \multiline{%
                    \textit{leading matrix}$[:,j]\gets$ leading subcircuit entry}
                    \If{$i=1$}
                        \State \multiline{%
                        \textit{trailing matrix}$[j,:]\gets$ subcircuit $L[0]$ entry}
                    \Else
                        \State \textit{trailing matrix}$[j,:]\gets$\textit{data buffer}$[[e_r],[e_c]]$
                    \EndIf
                    \State $j\gets j+1$
                \EndFor
                \State \textit{contracted}$\gets$\textit{leading}$\times$\textit{trailing} \Comment{Section~\ref{sec:programming_techniques}}
                \State \textit{next data buffer}$[[e_r],[e_c]]\gets$\textit{contracted}
            \EndFor
            \State \textit{data buffer} $\gets$ \textit{next data buffer}
            \State $i\gets i+1$
        \EndWhile
    \end{algorithmic}
\end{algorithm}

This section introduces compute graph contraction for an efficient postprocessing.
The final reconstruction of the probability output of the uncut circuit requires taking the outer products among the subcircuits and sum over
either all (without sampling) or the most important (with optimal sampling in Algorithm~\ref{alg:arbitrary_sampling}) edge bases.
While a naive computation of Equation~\ref{eq:CutQC} can simply iterate over all the $4^K$ different edge bases,
the reconstruction quickly becomes the bottleneck for complicated circuits
as it incurs many repetitive vector multiplications.
This is because subcircuits in general do not connect with all the edges
and hence remain unchanged across many different edge bases.
Computing the overall output of a compute graph shares a similar flavor with tensor network contractions,
which have been widely used in classical simulations of quantum systems~\cite{vidal2003efficient,vidal2004efficient,schollwock2011density,verstraete2004matrix}.
Algorithm~\ref{alg:compute_graph_contraction} shows the complete compute graph contraction algorithm.

Figure~\ref{fig:compute_graph_contraction_example} shows an example compute graph with $4$ subcircuits and $10$ edges.
Subcircuit $1$ in the compute graph only has $4^5$ different entries as it only attaches to $5$ edges.
As a result, the same subcircuit $1$ entry exactly appears in $4^5$ summation terms, as there are a total of $10$ edges in the compute graph.

Compute graph contraction takes advantage of this fact and eliminates the redundant computations.
On a high level, compute graph contraction merges two subcircuits (nodes) into a single node in every step,
eventually merging the entire graph.
Since ``contracting'' two subcircuits only concerns the common edges in between them,
the order of the contraction and the sizes of the individual subcircuits greatly affect the overall overhead.
Compute graph contraction chooses an order that minimizes the number of floating point numeric operations.

The naive computation of Figure~\ref{fig:compute_graph_contraction_example} computes as:
\begin{equation}
    \begin{split}
    \sum_{e_{1-10}\in\{I,X,Y,Z\}^{10}}&p_1(e_{1-5})\otimes p_2(e_{1,6-9})\\
    &\otimes p_3(e_{2,3,6,7,10})\otimes p_4(e_{4,5,8,9,10})\label{eq:naive_compute}
    \end{split}
\end{equation}
where $p_1(e_{1-5})$ represents the output of subcircuit $1$ with the edges $1,2,3,4,5$ in some certain bases and so on.
This reconstruction computes $4^{10}$ summation terms,
each requires $2^7+2^{14}+2^{25}$ floating point multiplications and $2^{25}$ floating point additions.
There are altogether roughly $10^{13.8}$ numeric operations.
Instead, Figure~\ref{fig:contraction_step_1} shows that first contracting the subcircuits $2$ and $3$ together transforms Equation~\ref{eq:naive_compute} into
\begin{equation}
    \begin{split}
    \sum_{e_{1,2,3,4,5,8,9,10}}&p_4(e_{4,5,8,9,10})\otimes p_1(e_{1,2,3,4,5})\\
    &\otimes\sum_{e_{6,7}}p_2(e_{1,6,7,8,9})\otimes p_3(e_{2,3,6,7,10})\label{eq:contract_step_1}
    \end{split}
\end{equation}
Equation~\ref{eq:contract_step_1} first computes the $4^6$ different summations between $p_2$ and $p_3$.
Each summation term is a matrix product between
the leading matrix from subcircuit $2$ of shape $(2^1,4^2)$
and the trailing matrix from subcircuit $3$ of shape $(4^2,2^7)$.
Figure~\ref{fig:contraction_step_2} shows that further contracting the subcircuit $1$ into the contracted subcircuits gives
\begin{equation}
    \begin{split}
        \sum_{e_{4,5,8,9,10}}&p_4(e_{4,5,8,9,10})\otimes\sum_{e_{1,2,3}}p_1(e_{1,2,3,4,5})\\
    &\otimes\sum_{e_{6,7}}p_2(e_{1,6,7,8,9})\otimes p_3(e_{2,3,6,7,10})\label{eq:contract_step_2}
    \end{split}
\end{equation}
Equation~\ref{eq:contract_step_2} then computes the $4^5$ different summations between $p_1$ and the previously merged $p_{2,3}$.
Each summation term is a matrix product between
the leading matrix from subcircuit $1$ of shape $(2^6,4^3)$
and the trailing matrix from subcircuits $2,3$ of shape $(4^3,2^8)$.
Figure~\ref{fig:contraction_step_3} shows that the last step eventually contracts $p_4$ with the previously contracted $p_{1,2,3}$.
This is a single matrix product between
the leading matrix from subcircuit $4$ of shape $(2^{11},4^5)$
and the trailing matrix from subcircuits $1,2,3$ of shape $(4^5,2^{14})$.
The entire process hence requires
\begin{equation*}
    \begin{split}
    &(4^2-1)\times 2^{8}\times 4^6+\\
    &(4^3-1)\times 2^{14}\times 4^5+\\
    &(4^5-1)\times 2^{25}\times 4^0
    \end{split}
\end{equation*}
additions and a similar number of multiplications, altogether roughly $10^{10.9}$ numeric operations.
Compute graph contraction for this particular example hence provides about $1000X$ compute overhead reduction.
The contraction order $3,2,1,4$ in fact minimizes the overhead for this example.

The contraction order of the subcircuits only affects the reconstruction up to a permutation of the qubit order,
and has no effect on the quantum state probability accuracy.
However, finding the optimal contraction order for general compute graphs is hard.
In fact, it is an active area of research and of broader interest across many disciplines~\cite{robertson1991graph,markov2008simulating,orus2014practical,gray2021hyper}.
In practice, quantum circuit cutting mostly incurs only several subcircuits.
This allows an exhaustive search over all the contraction orders to calculate the exact number of floating point operations required for each.
The experiments in this paper show that this searching process takes a negligible amount of time.
